Distance-based Positive and Unlabeled Learning for Ranking

Learning to rank -- producing a ranked list of items specific to a query and with respect to a set of supervisory items -- is a problem of general interest. The setting we consider is one in which no analytic description of what constitutes a good ranking is available. Instead, we have a collection of representations and supervisory information consisting of a (target item, interesting items set) pair. We demonstrate analytically, in simulation, and in real data examples that learning to rank via combining representations using an integer linear program is effective when the supervision is as light as "these few items are similar to your item of interest." While this nomination task is quite general, for specificity we present our methodology from the perspective of vertex nomination in graphs. The methodology described herein is model agnostic.

==> nd_text/nd_conclusion.tex <==
\section{Conclusion}
We have presented an integer linear programming solution for learning to rank via combining representations.
This task is
of general interest, but for specificity we have presented our methodology and results from the perspective of vertex nomination in graphs.
The results presented herein -- analytic, simulation, and experimental -- demonstrate that this methodology is principled, practical, and effective.
Our methodology makes essentially no model assumptions;
just that we are given a query item,
we know the dissimilarity (from multiple perspectives) between it and a set of items to be ranked,
and we have a set of items known to be similar to the query.

The three experimental settings highlight three complementary aspects of our vertex nomination problem.
In the first -- dMRI -- the issue is how to utilize two different spectral embedding techniques (LSE and ASE) each known to uncover different graph structure \cite{Priebe5995,cape2019spectral}.
In the second -- Bing -- the issue is how to utilize a collection of pre-defined representations (Node2Vec, wherein optimal hyperparameter settings are unavailable at embedding-time, and in any event no one setting will be optimal for all tasks) for multiple post-embedding nomination tasks.
In the third -- {\it Drosophila} -- the issue is how to utilize multiple different graphs (in this case, synapse types) each on the same vertex set.
In all three settings, the ILP solution successfully optimizes our ``learning to rank'' objective function to obtain a winning solution.

==> nd_text/nd_introduction.tex <==
\section*{Introduction} Given a query, a collection of items, and supervisory information, producing a ranked list relative to the query is of general interest. 
% \dropcap{G}iven a collection of items and a query item of particular interest together with supervisory information in the form of other related items, producing a useful ranked list of items specific to the query item and with respect to the supervisory items is of general interest.
In particular, learning to rank \cite{liu2009learning} and algorithms from related problem settings \cite{conte2004thirty} have been used to improve popular search engines and recommender systems and, impressively, aid in the identification of human traffickers \cite{fishkind2015vertex}.

When learning to rank, for each training query researchers typically have access to (feature vector, ordinal) pairs that are used to learn an ordinal regressor via fitting a model under a set of probabilistic assumptions \cite{robertson2009probabilistic} or via deep learning techniques \cite{severyn2015learning} that generalize to ranking items for never-before-seen queries. A query is an element of a set of possible queries $ Q $ and the items-to-be-ranked are elements of a nomination set $ \mc{N} $.

In this paper we consider the setting in which, for a given query, we know the dissimilarity (from multiple perspectives) between it and a set of items to be ranked. We are also given a set of items known to be similar to the query (positive examples). 
We make no model assumptions.
Our goal is to leverage the knowledge of the items known to be similar to the query to produce a new dissimilarity tailored to the query that is then useful for nominating items unknown to be similar to the query. The new dissimilarity is exactly a linear combination of the different dissimilarites, or representations, of the data and can gainfully be seen as combining representations to improve inference
\cite{vogelstein2020general}.
In the language of graphs:
with respect to a specific vertex of interest,
and given a set $S$ of important vertices and a collection of dissimilarity measures,
we solve an integer linear program that weights those dissimilarities so that the set of points in $S$ are ranked minimally;
we then use that learned weighted representation to rank all other vertices.
In short, we infer an entire ranking from light supervision in the form of the set $S$.


Related to our work, Fagin \cite{fagin1999combining} and the corresponding literature \cite{fagin2002combining} deal with a multi-media system (a system consisting of many subsystems) where the multi-media query $v^{**}$ is a boolean function of different $v^*_{1}$, $v^{*}_{2}, .. v^{*}_{m}$ 
with $v^{*}_{i}$ a query corresponding to subsystem $i$. Each subsystem is assumed to be able produce a ranked list for its corresponding query using fuzzy logic. In the context of our discussion, it is fruitful to think of these ranked lists as coming from different (marginal of subsystem $i$) representations of $v^{**}$. Fagin proposes an optimal algorithm for combining these representations under a set of assumptions --  most notably that the boolean function that combines the subsystem queries is known and that the subsystems are independent. These two assumptions, in particular, imply that supervisory information is not necessary. In our setting we make no assumptions on the structure of the query nor on the relationship between the representations and hence rely on supervisory information to combine representations.

While our set up is quite general, we study it through the lens of vertex nomination \cite{JMLR:v20:18-048}.

% \dropcap{T}he purpose of this paper is to introduce a methodology for learning a personalized "truth" for subsequent discovery.
%
%	"a methodology for learning an effective nomination representation for subsequent discovery by combining extant metric representations"
%
%In many modern data science applications,

% \dropcap{T}he purpose of this paper is to introduce a methodology for learning a personalized "truth" for subsequent inference specifically related to a given item of interest. Nomination of other items of potential interest is the goal,
% % Nomination of items of potential interest is the goal, 
% and the setting is one in which no analytic description of what is meant by interesting is available but an example consisting of a (target item, interesting items set) pair is available.
% This nomination task is of general interest, but for specificity we present our methodology from the perspective of vertex nomination in graphs.
% We demonstrate learning to rank via an integer linear program when the supervision is as light as "these few items are similar to your item of interest."


%LIT REVIEW !!!!!

\section*{Problem Description: Vertex Nomination}

In the single graph vertex nomination problem %\cite{coppersmith2014vertex}
\cite{JMLR:v20:18-048}
we are given a graph $ G = (V, E) $ and a single vertex of interest $ v^{*} \in V $,
and the task is to find other interesting vertices.
The vertex set $ V $ can be taken to be 
$V = [n] = \{1, \hdots, n\} $
%without loss of generality.
and the edge set $ E \subset {{V}\choose{2}}$ is a subset 
%-- directed or undirected -- 
of all possible vertex pairs $\{i,j\}$ with $ i, j \in [n] $.
The objective of vertex nomination is to return a ranked list of the candidate vertices $ V \setminus \{v^{*}\} $ such that ``interesting'' vertices
-- vertices ``similar'' to $ v^{*} $ --
are ranked high in this nomination list. Note that in vertex nomination the query set $ Q $ is $ \{v^{*}\} $ and the nomination set $ \mc{N} $ is $ V \setminus \{v^{*}\} $.
% Typically, vertex nomination proceeds under some application-specific notion of similarity/interestingness.

%[WHAT IS THIS?]
%Let $ \mc{S} \subseteq V $ denote the set of vertices similar to $ v^{*} $. 

%Typically, vertex nomination is an unsupervised learning problem because the definition of "similar" is unknown. 
Vertex nomination is a special case of (typically) unsupervised problems addressed by recommender systems \cite{bobadilla2013recommender} where it is assumed that {\it "[i]nformation relevant to the task is encoded in both the structure of the graph and the attributes on the edges"} \cite{coppersmith2014vertex}. There have been numerous approaches to vertex nomination proposed in recent years \cite{marchette2011vertex, coppersmith2012vertex, sun2012comparison, suwan2015bayesian, fishkind2015vertex, agterberg2019vertex, yoder2020vertex} with each illustrating success in sometimes adversarial settings. 

Notably, none of these proposed nomination schemes is universally consistent. Recall that a universally consistent decision rule is one where the limiting performance of the decision rule is Bayes optimal for every possible distribution of the data. In the classification setting, for example, the famed $ K $ Nearest Neighbor rule \cite{fix1951discriminatory}, with appropriate restrictions on $K$ growing with training set size, is in a class of decision rules known to be universally consistent \cite{stone1977consistent}, \cite[Chapters~5,6]{devroye2013probabilistic}. In their foundational paper on the theoretical framework of vertex nomination, Lyzinski et al.\ prove that there does not exist a universally consistent vertex nomination scheme \cite{JMLR:v20:18-048}. Their paper complements other theoretical \cite{peel2017ground} and empirical \cite{Priebe5995} results on the limitations of machine learning for popular unsupervised learning problems on graphs. The successes reported in \cite{marchette2011vertex, coppersmith2012vertex, sun2012comparison, suwan2015bayesian, fishkind2015vertex, agterberg2019vertex, yoder2020vertex} were all with respect to some application-specific notion of similarity/interestingness. 

In this paper,
in contrast to being told what is to be meant by similarity/interestingness,
we consider the setting in which, 
in addition to $ G $ and $ v^{*} $, 
we are given a set of vertices $ S \subset (V \setminus \{v^{*}\}) $ explicitly known to be similar to $ v^{*} $
from which we are to 
{\it learn} 
a ranking scheme
specific to the task at hand.
%We can leverage this information to improve nomination schemes.
In particular, we develop a nomination scheme $ f $ that takes as input $(G,v^*,S)$ -- a graph, a vertex of interest, and a set of vertices known to be similar to the vertex of interest --
and outputs a function that maps each vertex
not equal to $ v^{*} $ to an element of the set $ [n-1] $. 
% in the candidate set $C = V \setminus (\{v^*\} \cup S)$ to an element of the nomination range $R = [n-1-|S|]$. 
(We ignore the possibility of ranking ties for expediency;
see Appendix B.1 of \cite{JMLR:v20:18-048} for a discussion.)


We consider $S^* \subset (V \setminus \{v^*\})$
to be the collection of vertices that are truly similar to $v^*$;
thus the given supervisory set $S \subset S^*$
and the set $(S^* \setminus S)$,
% \subset C$, 
representing an unknown truth,
consists of vertices that we actually want to identify as interesting by placing them highly in the nomination list.
%-- are the elements of $(S^* \setminus S) \subset C$.
Letting $ \mc{H} = \{h: V \setminus \{v^{*}\} \to [n-1]\} $ be the set of functions, or rankers, that map a vertex to an element of $ [n-1] $ and $ \mc{G}_{V} $ be the set of graphs with vertex set $V$, a nomination scheme is a mapping $ f: \mc{G}_{V} \times V \times 2^{V} \to \mc{H} $. Our goal is to use an $ f $ such that $ f(G, v^{*}, S) = h(\cdot) $ outputs small values for elements of $S^* $.
% \setminus S$. 

We refer to the set $ C = (V \setminus (\{v^*\} \cup S)) $ as the candidate set and note that $ (S^{*} \setminus S) \subset C $.
For evaluation purposes it is convenient to consider the set of rankers that map from $ C $ to the nomination range $ R = [n-1-|S|] $. When there is a possibility of confusion we denote such rankers as $ h_{C} $, with $ \mc{H}_{C} = \{h_{C}: C \to R\} $. For every ranker $ h \in \mc{H} $ there is a ranker $ h_{C} \in \mc{H}_{C} $ such that $ h_{C}(v) $ is equal to $ h(v) $ minus the number of elements of $ S $ ranked higher than $ v $ in the nomination list induced by $ h $ for all $ v \in C $.

==> nd_text/nd_methods.tex <==
% \clearpage
\section{Methods}

\subsection{Natural Nomination, Given a Dissimilarity}

% \begin{comment}
% HH:\\
% Recall that $ h $ is a mapping from the candidate set $ C $ to the nomination range $ R $. Given a distance $ d^{j} $ a natural $ h $ to consider is the one that, given a vertex $ x_{v} $ in the candidate set, returns the rank of the distance (in ascending order) of the real number $ d(x_{1}, x_{V}) $. That is, the vertex in the candidate set closest to the vertex of interest in terms of distance $ j $ is mapped to 1. The vertex farthest from the vertex of interest in terms of distance $ j $ is mapped to $ n - 1 - |S| $. We let $ h^{j} $ denote the mapping from the vertex set to the distance rank for $ d^{j} $.
% \end{comment}

%cep:\\
Recall that $ h $ is a mapping
from the set of vertices minus $ v^{*} $ to the set of ranks $ \{1, \hdots, n - 1\} $.

%from the candidate set $ C $ to the nomination range $ R $. 
%Let $ x_{i} $ be a representation of vertex $ i $ in $ \mc{X} $. Given a distance $ d: \mc{X} \times \mc{X} \to \mbb{R}_+$, 
Given a dissimilarity measure $ d: V \times V \to \mbb{R} $,
a natural ranking function to consider is one that, given a vertex $v \neq v^{*} $, returns the rank 
% (in ascending order) 
% of the dissimilarity 
of the real number $ d(v^*,v) $ amongst the collection $\{d(v^*,v')\}_{v' \neq v^{*}}$.
That is, the vertex $ v \in (V \setminus \{v^{*}\}) $ that minimizes $ d(v^{*}, v) $
% closest to the vertex of interest 
is mapped to 1 -- the top of the nomination list -- and the vertex farthest from the vertex of interest is mapped to $ n - 1 $. 
We let $ h^d $ denote this mapping from the vertex set to the set $ [n-1] $ for dissimilarity $ d $.

We emphasize that throughout our discussion $ d $ need not satisfy the symmetry, triangle inequality or non-negativity requirements of a metric.

% NB: The "distances" we consider throughout need only be dissimilarities -- we do not need the triangle inequality.
% Rewrite

%{\color{red}[AB writes: We do NOT need any "metric" property. Certainly not the  "triangle inequality". We just need real valued weights (possibly even negative) to be able to sort.]}

%{\color{red}[We ignore the issue of distance ties, for expediency.]}

%{\color{blue} HH to CEP: i think i addressed the distance remark and the dissimilarity remark}

%Note that when the context strongly implies a particular representation we write $ d(v, v^{*}) $ instead of $ d(x_{v}, x_{v^{*}}) $.


%[AB 02/29/20, lighly edited by cep]
\subsection{An Integer Linear Program} \label{subsec:IP}

We present an optimization problem whose solution is useful for learning to rank in general and supervised vertex nomination in particular. 
Let $\{v_1, \ldots, v_n\}$ be a finite set of items.
% We are given a finite set of items which we denote by $\{v_1, \ldots, v_n\}$.
Without loss of generality we identify $v_1=v^*$.
%$\{v_0, v_1, \ldots, v_n\}$. 
We have a collection of $J$ distinct dissimilarity measures $ \{d^{1}, d^{2}, \hdots, d^{J}\} $ and have knowledge of the dissimilarity between $v_1$ and $v_i$, $i=2, \ldots, n$ for each of these measures. We use $d^j(v_{1}, v_{i}) $ to denote the dissimilarity between $v_1$ and $v_i$ in the $j$-th dissimilarity, $j=1, \ldots, J$. We are given a set $S \subset \{v_2, \ldots, v_n\}$ that we want to rank as high as possible by choosing an appropriate weighted combination of the $J$ dissimilarities. More precisely, we wish to select a set of weights $\alpha_1, \ldots, \alpha_J \geq 0$ such that when the elements $v_2, \ldots, v_n$ are ranked according to the dissimilarity $\alpha_1d^1(v_{1}, v_{i}) + \ldots + \alpha_Jd^J(v_{1}, v_{i})$ (for $i=2, \ldots, n$), the elements of $S$ are as close to the top of the ranked list as possible. 

Formally, for a given tuple of weights $\alpha = (\alpha_1, \ldots, \alpha_J)$, let %$rank_\alpha(v_i)$ 
$ h^{\alpha}(v_{i}) $ denote the rank of $v_i$ under the dissimilarity $\alpha_1d^1(v_{1}, v_{i}) + \ldots + \alpha_Jd^J(v_{1}, v_{i})$. We wish to solve the following optimization problem: \begin{equation}\label{eq:main-prob}
\min_{\alpha \geq 0} \;\; \max_{v \in S} \;\; %rank_\alpha(v)
h^{\alpha}(v).
\end{equation} 

The above problem can be formulated using the framework of {\it integer linear programming} (ILP). An ILP problem is an optimization problem where one wishes to minimize/maximize a linear function of a finite set of decision variables subject to linear inequality constraints and where a subset of the variables are required to take only integer values. In our current setting, we model~\eqref{eq:main-prob} as follows.

\begin{enumerate}
\item Introduce real valued decision variables $\alpha_1, \ldots, \alpha_J$ that are constrained to be nonnegative. These are the weights we are seeking in~\eqref{eq:main-prob}. We also impose the normalization constraint that $\alpha_1 + \ldots + \alpha_J = 1$, since scaling the weights by the same positive factor yields the same solutions.
\item Introduce {\it integer} variables $x_v$ for each item $v \not\in S$. Impose the linear constraints $0 \leq x_v \leq 1$; this forces $x_v \in \{0,1\}$ in any feasible solution. These variables are to be interpreted as follows: if $x_v=0$ in any solution, then $v$ is ranked worse than every element of $S$ (under $\alpha$) and if $x_v =1$ in any solution, then $v$ is ranked better than at least one element in $S$ (under $\alpha$).
\item The linear objective function involves only the $x_v$ variables: we wish to minimize $\sum_{v \not\in S} x_v$, because this sum equals the number of elements that are ranked better than at least one element of $S$ and thus captures the objective in~\eqref{eq:main-prob}.
\item We impose the linear constraints
\begin{align*}
\sum_{j=1}^{J} \alpha_{j} d^{j}(v_{1}, s) \leq \sum_{j=1}^{J} \alpha_{j} d^{j}(v_{1}, v) + M\cdot x_v \\ 
\;\; \forall (s, v) \in (S, C) \end{align*}
where $M := \max_{i, j} d^j_i$. This constraint imposes the desired condition that for any $v \in C $, if $x_v = 0$, then $v$ should be ranked worse than every element in $S$, i.e., its dissimilarity (under $\alpha$) from $v_1$ should be greater than or equal to the dissimilarity of every element of $S$ from $v_1$. If $x_v = 1$, then since $M$ is chosen to be the maximum of all possible dissimilarities and the coefficients $\alpha_1, \ldots, \alpha_J$ sum to 1, the constraint becomes a trivial constraint that is satisfied by all such nonnegative $\alpha$ values. 
Since we are minimizing $\sum_{v\not\in S}x_v$, for any $\alpha$, if an element $v\not\in S$ is ranked worse than every element of $S$, then the optimization would set $x_v$ to $0$. Thus, in any optimal solution $\alpha^*, x^*$ to the integer program, $x^*_v = 1$ if and only if $h^{\alpha^*}(v) < h^{\alpha^*}(s)$ for some $s\in S$.
\end{enumerate}

Once the problem~\eqref{eq:main-prob} is set up as an ILP as described above, one can bring state-of-the-art algorithms and software that employ a suite of sophisticated ideas borrowed from convex geometry, number theory and algorithm design to bear upon the problem. We have employed the commercial software Gurobi \cite{gurobi} to solve our ILP problems, which is among the most efficient and finely tuned software packages currently available for solving large scale ILPs. Open source alternatives to Gurobi include Common Optimization INterface for Operations Research (COIN-OR) \cite{lougee2003common} and SCIP: Solving Constraint Integer Programs \cite{achterberg2009scip}.

We note that the computational complexity of the proposed ILP is a complicated function of the number of vertices, the collection of representations 
%and distances 
considered, and the vertices $S$ known to be similar to the vertex of interest $ v^{*} $. 
In general, when the worst ranking element of $ S $ is ranked sufficiently poorly then the ILP is computationally burdensome. This issue is compounded when more than one element of $S$ is ranked poorly.


\subsection{The Solution Nomination List}

The $\alpha^*$ given by the solution to the integer program induces a dissimilarity $d^* = \sum_{j=1}^k \alpha^*_j d^j$, and the resultant $h^{d^*}$ provides an nomination list learned for $v^*$ from $ S$. We note that the ranker induced by $ d^* $ is not necessarily unique and is an element of the set $ \mc{H}^{*} = \{h: h \text{ minimizes } \eqref{eq:main-prob}\} $ whose constituent deciders map the elements of $ S $ close to the top of a nomination list.


\begin{comment}

\subsection*{HH}

Our goal, given a vertex of interest $ v^{*} := 1 $, a set of vertices $ S \subseteq \{2, .., n\} $, and a personal dissimilarity matrix 

\begin{align}
\Delta = \begin{bmatrix} 
d^{1}(x_{1}, x_{1}) & .. & d^{J}(x_{1}, x_{1}) \\
\vdots & \ddots & \vdots \\
d^{1}(x_{1}, x_{n}) & .. & d^{J}(x_{1}, x_{n})
\end{bmatrix}
\end{align} is to construct a dissimilarity $ \widehat{d}^* = \sum \alpha_{j} d^{j} $ with $\alpha_j > 0$ for all $j$ and $ \sum \alpha_{j} = 1 $ such that $ \widehat{d}^*(x_{1}, x_{s}) $ is "small" for a the unknown elements of $ S^{*} $. Assuming that the $ x_{s} $ are "similar" to the elements of $ S $, to find $ \widehat{d}^* $ we propose find the dissimilarity $ \widehat{d}^* $ that minimizes
\begin{align*}
    \max_{v \in S} \widehat{h}*(v)
\end{align*} where $ \widehat{h}^* $ is the mapping from the vertex set to the dissimilarity rank for $ \widehat{d}^* $. To find $ \widehat{d}^* $ we propose the following Integer Program (IP; implemented using Gurobi):

% Let $ V = \{1, \hdots, n\} =: [n]$. Define $ r_{(k)}^{j}(v^{*}) \in V \setminus \{v^{*}\} $ to be $ v^{*} $'s $ kth $ nearest neighbor as defined by distance $ j $. Further, let $ R^{j}(v) = [r_{(1)}^{j}(v^{*}), .., r_{(n)}^{j}(v^{*})] $ be the list of vertices ranked according to their distance to $ v $ in embedding $ j $ and the function $ p^{j}_{v^{*}}: V \setminus \{v^{*}\} \to [n-1] $ be the mapping from the reduced vertex set to its rank. To find $ d^{*} $ we find a linear combination of the $ \{d^{j}\} $ such that 
% \begin{align} \label{goal}
% \max_{v \in S} p_{v^{*}}^{*}(v) 
% \end{align} is minimized,
% where $p^*$ is defined as the analog of $p^j$ for the optimal linear combination of the $J$ distances.

Recall that the candidate set $ C $ contains the vertices that are not the vertex of interest nor an element of S. For a fixed dissimilarity $ d' = \sum \alpha_{j}' d^{j} $, $ C $ can be decomposed into two disjoint subsets, $ C_{+}' $ and $ C_{-}' $, where $ v' \in C_{+}' $ is such that $ h'(v') < \max_{v \in S} h'(v) $. That is, for a given $ v^{*}, S $ and $ d' $, the vertices in $ C_{+}' $ are those that are higher in the nomination list than the vertex in $S$ that is lowest on the list. Intuitively, we want to find a dissimilarity such that the cardinality of $ C_{+}' $ is smallest -- meaning most of the vertices in $S$ are high in the nomination list.

Define $ c' $ to be the binary vector of length $ |C| $ where a $ 1 $ in the $ith$ index 
corresponds to the $ ith $ vertex of $C$
being in $ C_{+}' $. Let $ M = \max \Delta_{ij} $. Then $ \widehat{d}^{*} $ is such that
\begin{align*}
\sum_{v \in C} c'_{v}
\end{align*} 
is minimized subject to the constraints
\begin{gather}\label{linear-constraints}
\sum_{j=1}^{J} \alpha_{j} d^{j}(v^{*}, s) \leq \sum_{j=1}^{J} \alpha_{j} d^{j}(v^{*}, v) + c'_{v} M \\ \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \forall (s, v) \in S \times C \nonumber \\
\sum_{j=1}^{J} \alpha_{j} = 1
\\
\alpha_j \geq 0, j = 1, \ldots, J
\\
c_k \in \{0,1\}, k=1,\ldots, |Q|
\end{gather}

The decision variables are the $\alpha_j$ and the $c_k$.
The set of constraints implied by Equation \ref{linear-constraints} ensure that the new dissimilarity $ d' $ places the elements of $ S $ below the elements of $ C_{+}' $ and above the elements of $ C_{-}' $ in the nomination list. These constraints are decomposed into two terms. The second term, $ c'_{j} M $, makes the constraint trivially satisfied when $ j \in C_{+}' $. For elements of $ C $ not in $ C_{+}' $ the new dissimilarity between it and $ v^{*} $ must be larger than the dissimilarity between any element of $ S $ and $ v^{*} $. 

Note that the IP takes as input a subset of vertices $ S $ and a dissimilarity matrix $ \Delta $.

\end{comment}

\subsection{Comparing two rankers}

% Let $ f $ and $ f' $ be two nomination schemes and $\ell $ be a loss function $ \ell: [n-1-|S|] \to \mbb{R}_{+} $ such as mean reciprocal rank.

% Given $ G, v^{*}$ an $ S $, define the \textit{risk} of $ f(G, v^{*}, S) = h(\cdot) $, $ R(h) $, to be the average loss of $ h(s) $, with $ s \in \mc{S} \setminus S $. We say $ f $ is better than $ f' $ for a given $ (G, v^{*}, S) $ if $ R(f) < R(f') $.

% Now, let $ (G, v^{*}, S) \sim F_{G,v^{*},S} $. The generalization error of $ f $, $ \mc{E}(f) $, is defined as the \textit{expected risk} of $ f $. Formally,
% \begin{align*}
    % \mc{E}(f, F_{G,v^{*},S}) = \mbb{E}_{F}\left[\mbb{E}_{\mc{S} \setminus S}\left(R(f(G, v^{*}, S)\right)\right].
% \end{align*} We say $ f $ is better than $ f' $ for a given $ F_{G,v^{*},S} $ if $ \mc{E}(f) < \mc{E}(f') $. Often, the graph $ G $ is fixed and we want to compare nomination schemes for various $ (v^{*}, S) $ pairs. In this case we can simply consider $ \mc{E}(f, F_{v*, S | G=g}) $.

In the simulations and real data experiments below we compare nomination schemes using Mean Reciprocal Rank (MRR). MRR is one of many measures commonly used in information retrieval to evaluate a nomination list for a given set of objects \cite{radev2002evaluating}. Let $ h $ be a ranker and $ \mc{N}' $ be a subset of the nomination objects $ \mc{N} $. The MRR of $ h $ for $ \mc{N}' $ is the average of the multiplicative inverse (or reciprocal) of the $ h(s) $ for $ s \in \mc{N} $. That is,
\begin{align*}
    \text{MRR}(h, \mc{N}') = \frac{1}{|\mc{N}'|}\sum_{s \in \mc{N}'} \frac{1}{h(s)}.
\end{align*} For a given $ \mc{N}' $ and two rankers $ h $, $ h' $, the ranker $ h $ is preferred to the ranker $ h' $ for $ \mc{N}' $ if $\text{MRR}(h, \mc{N}') > \text{MRR}(h', \mc{N}')$. 
%If the size of $ Q $ is 1 then we call Mean Reciprocal Rank simply Reciprocal Rank.


\section{A Generative Model Example}

% Add a sentence about latent position graphs (Hoff, Raftery and Hancock)

Latent space network models \cite{hoff2002latent} are random graph models where each vertex has associated with it a latent vector and the probability of an edge between two vertices is determined by a function of two vectors, typically called a \textit{kernel}. One such latent space model is the Random Dot Product Graph (RDPG) where the kernel function is the inner product \cite{athreya2017statistical}.

We consider latent positions $ X_{1}, .., X_{n} \iid F $ on $\mbb{R}^m$ 
associated with the vertices
$v_{1}, .., v_{n}$
where the distribution $ F $ is such that  
$0 \le \langle x,y \rangle \le 1 $
for all $x,y$ in the support.
%for $ X, Y \in \mathbb{R}^{d} \iid F $ $ 0 \le \langle X, Y \rangle \le 1 $. 
Let $ X $ denote the $n \times m$ matrix with the $X_{i}$'s as rows. That is,
\begin{align*}
X = \begin{bmatrix} X_{1}^{\T} \\ \vdots \\ X_{n}^{\T} \end{bmatrix}.
\end{align*}
Then $ P = X X^{\T}$ is the $n \times n$ RDPG connectivity probability matrix.
Let $ T^{1}, \hdots, T^{J} $ be different embedding functions; that is, each $T^j: \mathcal{M}_n \to (\mbb{R}^{m_{j}})^n$ takes as input an $ n \times n $ matrix and outputs $ n $ points in $\mbb{R}^{m_{j}}$. For example, the adjacency spectral embedding of $ P = U_{P} \Sigma_{P} U_{P}^{\T} $ is an embedding with $ T_{ASE}(P) = U_{P}|\Sigma_{P}|^{1/2} $. We let $ T(P)_{i} $ denote the representation of node $ i $ resulting from the transformation $ T $. 
Then $ T_{ASE}(P)_{i} = X_{i} $ (up to an orthogonal transformation).
% {\color{red}Amitabh: Up to an orthogonal transformation?}. 
Further suppose that with each embedding function comes a dissimilarity $ d^{j}: \mbb{R}^{m_{j}} \times \mbb{R}^{m_{j}} \to [0, \infty) $. This induces a $v_1$-specific ``personal'' dissimilarity matrix
\begin{align*}
\Delta_{v_{1}} = 
    \begin{bmatrix} 
        d^{1}(T^{1}(P)_{1}, T^{1}(P)_{1}) & .. & d^{J}(T^{J}(P)_{1}, T^{J}(P)_{1}) \\
        \vdots & \ddots & \vdots \\
        d^{1}(T^{1}(P)_{1}, T^{1}(P)_{n}) & .. & d^{J}(T^{J}(P)_{1}, T^{J}(P)_{n})
    \end{bmatrix}
\end{align*} containing the dissimilarities from the (representation of the latent position for) the vertex of interest 
%$v^{*}$ 
(without loss of generality, we are letting the vertex of interest be index 1: $v^*=v_1$) 
to every other vertex for every transformation in terms of its induced dissimilarity. Recall that the ILP takes as input a subset of vertices $S$ and a personal dissimilarity matrix $\Delta_{v^{*}}$.

As above, our goal is to construct a dissimilarity $ d' = \sum \alpha_{j} d^{j} $ with $ \sum \alpha_{j} = 1 $, $ \alpha_{j} \ge 0 $  such that $ d'(v_{1}, v_{s^{*}}) $ is "small"
%with high probability 
for the elements of $ (S^{*} \setminus S) $, the vertices truly, but unknown to be, similar to $ v^{*} $.


\subsection{An Illustrative Analytic Example}

We illustrate the geometry of combining representations in the
RDPG model
using Laplacian Spectral Embedding (LSE) and Adjacency Spectral Embedding (ASE)
\cite{von2007tutorial, sussman2012consistent}.

Given a particular realization of the $X_i$'s, $P$ is fixed (non-random).
We consider $x_1 = [0.5, 0.5]^{T}$
and 
$x_{2}, \hdots, x_{51}$ to be realizations from the uniform distribution on the positive unit disk in $ \mathbb{R}^{2} $.
We consider two embedding functions: $ T^{1}(P) = U_{P}|\Sigma_{P}|^{1/2} $ and $ T^{2}(P) = \sqrt{n}  U_{L(P)} |\Sigma_{L(P)}|^{1/2} $, both truncated at embedding dimension $ m = 2 $, where $ L(P) = D^{-1/2} P D^{-1/2}$ with $ D_{ii} $ equal to the $ i $th row sum of $ P $. The corresponding dissimilarities are taken to be Euclidean distance. 

Figure \ref{fig:example_latent} shows that the interpoint distance rankings induced by $ T^{1} $ (ASE) and $ T^{2} $ (LSE) are not necessarily the same, thus demonstrating the basis of the ``two truths" phenomenon in spectral graph clustering \cite{Priebe5995}. Further, the interpoint distance rankings from a linear combination of the two Euclidean distances is neither equal to the rankings from ASE nor the rankings from LSE.
This indicates that the solution found by the ILP 
% that solves \eqref{eq:main-prob} 
can produce a superior nomination list compared to either ASE or LSE alone. 

\begin{figure*}[ht]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \includegraphics[width=\textwidth]{images/simulation/your_truth_combined.pdf}
    % \begin{subfigure}[t]{0.32\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{images/example_latent_ASE.png}
    %     \caption{}
    % \end{subfigure}%
    % ~ 
    % \begin{subfigure}[t]{0.32\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{images/example_latent_LSE.png}
    %     \caption{}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.32\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{images/example_latent_both.png}
    %     \caption{}
    % \end{subfigure}
    \caption{Ranking of interpoint distances is not preserved across vertex representations. Each panel shows an embedding of the probability matrix $ P $, with LSE on the left, the induced embedding for $ \alpha=0.2 $ in the center, and ASE on the right. In each panel, 9 vertices are highlighted: 1) $v^{*}$ -- the vertex of interest $ v^{*} $; 2-6) $S$ -- the five vertices closest to $ v^{*} $ as defined by $ d_{0.2} = 0.2 d_{ASE} + 0.8 d_{LSE} $; and 7-9) $s^{*}_{LSE}, s^{*}_{0.2} $ and $ s^{*}_{ASE} $ -- the closest vertex to $ v^{*} $ that is not an element of $ S $ as defined by $ d_{LSE} $, $ d_{0.2} $ and $ d_{ASE} $, respectively. The number near each of the three $ s^{*} $ in each panel is the Euclidean distance between it and $ v^{*} $ for that particular embedding. Note that the ordering of these distances is not preserved across panels. This implies that inference based on the ranking of the interpoint distances is not invariant to the representation of the vertices.
    % The rankings induced by linear combinations of distances can differ. In all three panels a vertex of interest is red; the three vertices closest to the vertex of interest (as defined by $ \alpha d_{ASE} + (1-\alpha)d_{LSE} $ are gold; the closest non-gold point (as defined by $ \alpha d_{ASE} + (1-\alpha)d_{LSE} $) is green. The left panel shows points space induced by $ \alpha d_{ASE} + (1-\alpha)d_{LSE} $ found by cMDS. The center panel shows the ASE ($\alpha=1$) representation of the points. The closest non-gold point in the ASE representation is black. The right panel is the same for LSE ($\alpha=0$). 
    % The left panel sho shows $ v^{*} $, the $ |S| = 3 $ closest vertices to it, and $ s^{*} $ = the fourth closest vertex, as defined by the Euclidean distance on the $ T^{1}(P)_{i} $. Subfigure b) shows the same for the $ T^{2}(P)_{i} $. Subfigure c) is a combination of subfigures a) and b) and shows that the 3 closest vertices defined on two embeddings are not necessarily the same.
    }
    \label{fig:example_latent}
\end{figure*}

\subsection{An Illustrative Simulation Example}

In the RDPG setting we do not observe $ P $ directly. Instead, we observe an adjacency matrix $ A $ such that $ A_{ij} \stackrel{ind}{\sim} Bernoulli(P_{ij}) $ for $ i < j $, $ A_{ji} = A_{ij} $,
and $ A_{ii} = 0 $.
Note that, save for the diagonal,
$ P = \mbb{E}(A) $. 

Revisiting our analytic example,
with geometry illustrated in
Figure \ref{fig:example_latent},
we consider the setting in which we observe $ \bar{A} = \frac{1}{k} \sum_{i=1}^{k} A_{i} $ with $ A_{1}, \hdots, A_{k} \iid Bernoulli(P) $. We define ``interestingness" based on the dissimilarity $ d_{\alpha} = \alpha d_{ASE} + (1-\alpha) d_{LSE} $ where $ d_{\{A,L\}SE} $ is Euclidean distance defined on the vertices after embedding $P$ via \{A,L\}SE. We let $ S^{*} $ be the six closest vertices to $ v^{*} $ as defined by $ d_{\alpha} $ after embedding the true but unknown probability matrix $ P $. 



Figure \ref{fig:example_simulation} presents the results from this simulation set up for various values of $ \alpha $ where $ S $ is the set of five closest vertices to $ v^{*} $ as defined by $ d_{\alpha} $. The rankers are evaluated based on where the sixth closest element, $ s^{*} $, as defined by $ d_{\alpha} $, is in their respective nomination lists.
% The points labeled $ s^{*} \{LSE, alpha=0.2, ASE\} $ are the closest vertices not in $ S $ from the perspective of the three dissimilarity measures $ d_{LSE}, d_{0.2}, $ and $ d_{ASE} $. 
The left panel shows the performance of the ILP and rankers induced by $ d_{ASE} $ and $ d_{LSE} $ when the $ P $ matrix is observed. The right panel shows the performance of the same three schemes when $ k = 1000 $. Reciprocal rank is estimated using 100 Monte Carlo simulations. Shaded regions indicate the 95\% confidence interval for the mean. The two panels demonstrate
the utility of the ILP solution for learning to nominate in both noiseless and noisy settings. We note that when $ \alpha = 0 $ ``interestingness" coincides exactly with the dissimilarity defined on the representation of the vertices after embedding via LSE and that when $ \alpha = 1 $ ``interestingness" coincides exactly with the dissimilarity defined on the representation of the vertices after embedding via ASE.




\begin{figure}[ht]
    \centering
    \captionsetup[subfigure]{justification=centering}
        \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\linewidth]{images/simulation/mrr_nmc100_n50_d2_acorn18008_poc.pdf}
        \caption{}
        \label{subfig:simulation_P}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\linewidth]{images/simulation/mrr_nmc100_n50_d2_k1000_acorn18008.pdf}
        \caption{}
        \label{subfig:simulation_A}
    \end{subfigure}
%    \includegraphics[width=\columnwidth]{images/simulation/mrr_nmc50_n50_d2_k1000_acorn18008.pdf}
%    \includegraphics[width=\columnwidth]{images/simulation/mrr_nmc50_n50_d2_k1000_acorn18008.pdf}
    \caption{The proposed ILP demonstrates utility both analytically in the noiseless setting (left) and via simulation in the noisy setting (right). In both settings the definition of ``interestingness" is based on a linear combination of the distances induced by the adjacency and Laplacian spectral embeddings of the $ P $ matrix. The left panel shows the performance of the ILP and the rankers induced by ASE and LSE when the $ P $ matrix is observed. Notice that the performances of the ILP and LSE (resp.\ ASE) are the same when $\alpha$ = 0 (resp.\ 1);
    in these cases ``interestingness" coincides exactly with the distances induced by LSE and ASE. The right panel shows the performance of the same nomination scheme %when $ \bar{A} = \frac{1}{1000}\sum_{i=1}^{1000} A_{i} $ is 
    for observed graphs instead of $ P $. 
%A1, .., Ak iid P;
%Abar = $(1/k) \sum A_i$;
%Xhat = ASE(Abar);
%Xbreve = LSE(Abar);
%k=1000.
%in practice we do not know alpha.
%the "Bayes rank" for uniform prior on alpha ...
%averaging mean mrr over alpha:
%IP - 2.15;
%LSE - 3.14;
%ASE - 3.68.
% At $\alpha=0$ "truth" is ASE; at $\alpha=1$ "truth" is LSE.
% ILP solution is generally superior for $\alpha \in (0,1)$.
    }
    \label{fig:example_simulation}
\end{figure}


In general, it is possible that either ASE or LSE places $s^{*}$ at the top of their respective nomination lists for any given $ \alpha $. When this happens, as is the case for $\alpha=0.7$ for the latent positions described in Figure \ref{fig:example_latent}, finding a linear combination of weights that optimize \eqref{eq:main-prob} may not similarly place $s^{*}$ at the top of its corresponding nomination list. This happens, for example, when a representation that does not place $s^{*}$ at the top of its nomination list places the elements of $S$ closer to the top of its nomination list as compared to the representation that places $s^{*}$ at the top. Hence, per the objective function, the weight corresponding to the representation that does not place $s^{*}$ at the top will be larger and the performance of the ILP may suffer, as seen in Figure \ref{fig:example_simulation}.



%Indeed, $ A $ is a noisy observation of $ P $ with $ A_{ij} = P_{ij} + E_{ij} $ and $ E_{ij} = 1 - P_{ij} $ with probability $ P_{ij} $ and $ E_{ij} = - P_{ij} $ with probability $ 1 - P_{ij} $.

% Given $A$, 
% and with $v^*$ and $S$
% as in Figure Figure \ref{fig:example_latent},
% we consider "truth"
% to be given by some $\alpha$ (unknown outside of the simulation setting).
% %To find $ \widehat{d}^{*} $ 
% We construct a noisy version of the distance matrix $ \Delta_{v_{1}} $ described above
% \begin{align*}
% \hat{\Delta}_{v_{1}} = 
% \begin{bmatrix} d^{1}(T^{1}(A)_{1}, T^{1}(A)_{1}) & .. & d^{J}(T^{J}(A)_{1}, T^{J}(A)_{1}) \\
% \vdots & \ddots & \vdots \\
% d^{1}(T^{1}(A)_{1}, T^{1}(A)_{n}) & .. & d^{J}(T^{J}(A)_{1}, T^{J}(A)_{n})
% \end{bmatrix}
% \end{align*} and use $S$ and $ \hat{\Delta}_{v_{1}} $ as input to the ILP. 
% MRR
% (when the size of $ Q $ is 1 then we call Mean Reciprocal Rank simply Reciprocal Rank)
% shows that the ILP solution is generally superior.
% NB: at $\alpha=0$ "truth" is ASE; at $\alpha=1$ "truth" is LSE.



% \subsection*{Comparing two nomination schemes}

% Let $ f $ and $ f' $ be two nomination schemes and $\ell $ be a loss function $ \ell: [n-1-|S|] \to \mbb{R}_{+} $ such as mean reciprocal rank.

% Given $ G, v^{*}$ an $ S $, define the \textit{risk} of $ f(G, v^{*}, S) = h(\cdot) $, $ R(h) $, to be the average loss of $ h(s) $, with $ s \in \mc{S} \setminus S $. We say $ f $ is better than $ f' $ for a given $ (G, v^{*}, S) $ if $ R(f) < R(f') $.

% Now, let $ (G, v^{*}, S) \sim F_{G,v^{*},S} $. The generalization error of $ f $, $ \mc{E}(f) $, is defined as the \textit{expected risk} of $ f $. Formally,
% \begin{align*}
    % \mc{E}(f, F_{G,v^{*},S}) = \mbb{E}_{F}\left[\mbb{E}_{\mc{S} \setminus S}\left(R(f(G, v^{*}, S)\right)\right].
% \end{align*} We say $ f $ is better than $ f' $ for a given $ F_{G,v^{*},S} $ if $ \mc{E}(f) < \mc{E}(f') $. Often, the graph $ G $ is fixed and we want to compare nomination schemes for various $ (v^{*}, S) $ pairs. In this case we can simply consider $ \mc{E}(f, F_{v*, S | G=g}) $.

% In the real data analysis we compare two nomination schemes using Mean Reciprocal Rank ($ MRR $). $ MRR $  is commonly used in information retrieval to evaluate a nomination list for a given set of queries. Let $ h $ be a nomination scheme and $ Q $ a set of query vertices. The $ MRR $ of $ h $ for $ Q $ is the average of the multiplicative inverse (or reciprocal) of the $ h(q) $ for $ q \in Q $. That is,
% \begin{align*}
%     MRR(h, Q) = \frac{1}{|Q|}\sum_{q \in Q} \frac{1}{h(q)}.
% \end{align*} For a fixed $ Q $ and two nomination schemes $ h $, $ h' $, the scheme $ h $ is preferred to $ h' $ for the query set $ Q $ if $ MRR(h, Q) > MRR(h', Q) $


% Let $ V = [n] $ be a vertex set and $ \Xi_{n, v} $ be the set of all sequences that contain the integers $ 1, \hdots, n $, with the exception of $ v \in [n] $, all exactly once.  

% Given a vertex of interest, $ v^{*} := 0 $, the goal of vertex nomination is to produce a ranked list that places vertices similar to $ v^{*} $ near the top of the list. Note that the definition of similar may be dependent on $ v^{*} $. A nomination scheme $ \phi(\cdot) $ is a function that takes as input an element of the vertex set and outputs a sequence of the integers $ [n] \ v^{*} $. That is,  $ \phi: V \to \Xi_{n,v^{*}} $.

% For a collection of $ v^{*} $s it is natural to want to compare two nomination schemes $ \phi, \phi' $. In particular, for a collection of $ v^{*} $


% TODO@hh.

==> nd_text/nd_real_data.tex <==
\section{Real Data Examples}
We consider three real data examples:
diffusion MRI connectome, search navigation, and {\it Drosophila} connectome.

%\clearpage

\subsection{dMRI}

We consider a graph $G_{dMRI}$
% {\color{red}["DS72784-subj1-scan1-Xhat.RData"]}
from a collection of connectomes estimated using a diffusion MRI-to-graph pipeline \cite{Kiar188706}. Vertices represent subregions defined via spatial proximity and edges are defined by tensor-based fiber streamlines connecting these regions. %We start with 
%the pairwise distances between vertices in 
%the largest connected component of 
$ G_{dMRI} $ has $n = |V| = 40,813$ vertices and  $e = |E| = 2,224,492$ edges.

The vertices of $G_{dMRI}$ each belong to exactly one of $ 70 $ Desikan regions of the brain -- 35 anatomical regions in each of the two hemispheres \cite{desikan2006automated}. %Regions $ 2 - 36 $ correspond to Desikan anatomical regions in the left hemisphere. Regions $ 36 - 71 $ are the analogous regions in the right hemisphere. Region $ 1 $ is \{something\}. That is, for $ 2 \leq i \le 36 $, $ i $ and $ i + 35 $ denote the same region in the two hemispheres. 
%We let $ V_{i} $ be the subset of vertices in region $i$: .
%and let $ V_{i,j} = V_{i} \cup V_{j} $. 
Furthermore, each vertex also has a designation as either gray matter or white matter. 
%Within a region, vertices can be either gray or white matter.
Thus, each vertex has a region label, a hemisphere label, and a tissue type label.

We consider
 $ J = 2 $ spectral embedding representations of $G_{dMRI}$:
ASE (embedding dimension $m=15$) 
and LSE (embedding dimension $m=46$). 
In the illustrative paper \cite{Priebe5995}, aptly titled {\it On a two-truths phenomenon in spectral graph clustering}, it is demonstrated that these two representations 
%of $G_{dMRI}$, LSE \& ASE,
lead to two fundamentally different clusterings -- LSE best for the affinity structure associated with hemisphere (left vs.\ right) and ASE best for  the core-periphery structure associated with tissue type (gray vs.\ white).
That is, there are two truths,
and the two embeddings are each best for recovering a different truth.
In the conclusion to \cite{Priebe5995} %TT@PNAS2019,
the authors write
{\it ``For connectomics, this phenomenon [$\dots$] suggests that a connectivity-based parcellation based on spectral clustering should consider both LSE and ASE''}.  
The methodology developed herein allows just such an analysis.





%we sample vertices from $ V_{3, 3+35} $, the union of the $ 351 $ vertices from region $ 3 $ and the $ 395 $ vertices from region $ 3 + 35 $. 


% For this graph, the number of vertices $n = 40813$.
For illustration, we consider the target brain structure to be Desikan region "anterior cingulate cortex" (ACC).
%\cup V_{38}$.
The  vertex of interest $v^*$ is chosen at random from $V_{ACC}$,
and the remainder of vertices in $V_{ACC}$ are designated as $S^*$ -- truly similar to $v^*$.
%$|V_{3} \cup V_{38}| = 351 + 395 = 746$, 
$|V_{ACC}| = 746$,
so $|S^*| = 745$.
Then $S \subset S^*$ with $|S|=50$ is randomly chosen,
leaving
$|S^* \setminus S| = 695$ truly, but unknown to be, interesting vertices out of a candidate set 
$C = V \setminus (\{v^*\} \cup S)$ with 
$|C| = n-1-|S| = 40,762$.

%About $ 65\% $ of the vertices in Desikan region CMFG are white matter.
$V_{ACC}$
 includes vertices from both hemispheres and from both tissue types;
loosely speaking, the "truth" for $ v^{*} $, as exemplified by the characteristics of the elements of $ S $, is a combination of the original two truths. Hence, a nomination scheme that combines LSE and ASE promises superior nomination performance.

We compare the nomination schemes induced by the ASE and the LSE distances to the ILP nomination scheme that identifies an optimal linear combination of the two.

%The ILP runs on this large problem.
%{\color{red} NB: this took a week using GUROBI, serially for 150 (v*,S*) pairs, on HH's local machine.}
% Intel(R) Core(TM) i7-8650U CPU @ 1.90 GHz, 2112 MHz, 4 Core(s), 8 Logical Processor(s)
The competing nomination schemes are evaluated via MRR.
%the  Mean Reciprocal Rank (MRR) of the remaining elements of $ V_{3, 3+35} \setminus \{v^{*}\} \setminus S $.
We performed this ($v^*,S^*$) sampling a total of 150 times.
The paired differences between the MRR from the ILP and ASE and between the MRR from the ILP and LSE are depicted in Figure \ref{fig:ip_minus_dmri};
%and \ref{subfig:ip_minus_lse_dmri}, respectively; 
positive values indicate that the ILP performs better than its competitor.
Testing for a difference in the medians between ILP and \{ASE,LSE\}
%and between IP and LSE 
via Wilcoxon's signed rank test 
  % two-sided !!!!!
yields p-values 
%$p \approx 0.0113$ for ASE and 
%$p < 0.00001$ for LSE, 
$p \approx 0.0057$ for "H0: ASE as good or better than ILP" and 
$p < 0.00001$ for "H0: LSE as good or better than ILP", 
demonstrating a statistically significant improvement in nomination performance for the ILP solution.


\begin{figure}
    \centering
    \captionsetup[subfigure]{justification=centering}
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\linewidth]{images/dmri/ip_minus_ase_combined.pdf}
        \caption{}
        \label{subfig:ip_minus_ase_dmri}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\linewidth]{images/dmri/ip_minus_lse_combined.pdf}
        \caption{}
        \label{subfig:ip_minus_lse_dmri}
    \end{subfigure}
    \caption{For nominating the anterior cingulate cortex (ACC): histograms and kernel density estimates for the difference of paired Mean Reciprocal Ranks (MRR) between the nomination list induced by the Integer Linear Program (ILP) and the nomination list from ASE (a) and LSE (b). The vertex of interest $v^*$ and interesting vertex set $S$
    %, $ |S|=50 $, 
    were sampled 
    %without replacement 
    from $V_{ACC}$. 
    MRR was calculated using the remaining elements of $V_{ACC}$. 
    %Ties were removed. 
    %   IP win | tie | xSE win
    %ASE:   89 |  0  |  61
    %LSE:   71 | 48  |  31
    %pbinom(61,150,.5) 0.0135763
    %pbinom(31,102,.5) 4.653825e-05
    Qualitatively, both distributions of differences are inclined to the positive. Quantitatively, 
    %testing for symmetry about zero using 
    Wilcoxon's signed rank test yields p-values $ p \approx 0.0057 $ and $p < 0.00001$ for ASE and LSE, respectively,
    demonstrating a statistically significant improvement in nomination performance for the ILP solution.}
    \label{fig:ip_minus_dmri}
\end{figure}





%\clearpage

\subsection{Bing}

The second real data example we consider is derived from Microsoft's Bing search navigation data collected over the course of 2019. The search navigation data consists of pairs of queries that are submitted to Bing in succession by a user within a browsing session. We consider the pairs of queries that correspond to a preidentified list of products in consumer electronics, household appliances, and gaming.

We use this data to construct a graph where the edge weight between two products in the graph is a normalized count of the pairs of queries that contain the two products. We remove self-loops and edges with edge weights below a user-selected threshold and analyze only the largest connected component, $ G_{Bing} $. $ G_{Bing} $ has $ n = |V| = 7,876 $ vertices and $ e = |E| = 46,062 $ directed weighted edges. 
% We consider a graph $G_{Bing}$, an induced subgraph of [\textit{describe Bing data}], containing [WHAT VERTICES DID THEY KEEP]. The induced subgraph $ G_{Bing} $ has $ n = |V| = 7876 $ and $ e = |E| = $ NEDGES. 

We consider $ J = 100 $ different representations of $ G_{Bing} $. Each representation is a Node2Vec embedding \cite{grover2016node2vec} corresponding to different hyperparameter settings. 

% The $ 100 $ representations we consider are from a set of $ 100 $ Node2Vec representations. They were selected because the induced distances from the $ NREPS $ representations provide a covering of the entire set of $ 100 $. That is, for every representation not included in the $ NREPS $, the interpoint distances induced the the representation are ``sufficiently" close to the interpoint distances induced by one of the $ NREPS $ representations included.

% Each including ASE for various embedding dimensions, LSE for various embedding dimensions and power iterations \cite{mises1929praktische}, and Node2Vec  for various hyperparameter settings.

Along with the representations, we are given three vertices of interest. All three vertices of interest correspond to phones. For each vertex of interest $ v^{*} $, we are given a set of vertices $ S^{*} $ known to be similar to $ v^{*} $. These sets were handpicked by a team of data scientists at Microsoft. Each $ S^{*} $ contains 20 products. A product was included either because it is a phone produced by the same company and is sufficiently close in generation or because it is of the same generation but produced by a different company.

% To determine what ``sufficiently" close meant for the $ 100 $ representations, we calculated the $ {100 \choose 2} $ pairwise L2-norms of the differences of the distance vectors induced by the representations for each $ v^{*} $. We then sorted the $ 12 {100 \choose 2} $  L2-norms in descending order and deployed an ``elbow" finding technique \cite{zhu2006automatic}, typically used in problems requiring dimensionality reduction, to automatically select a covering threshold. That is, elbows in the plot of descending pairwise L2-norms loosely correspond to different levels of uniqueness amongst representations. The pairwise L2-norms are shown in the left panel of Figure \ref{fig:ip_minus_bing}.



% Once the covering threshold was chosen, representations were recursively added to a set of unique representations. In particular, for $ v^{*}_{1} $ we initialized the set of unique representations with the first representation and subsequently selected representations where the L2-norm between its induced distance vector and the induced distance vector of every element in the set of unique representations was above the covering threshold threshold. For $ v^{*}_{2} $ the set of unique distances was initialized with the set found using $ v^{*}_{1} $ and the process was repeated. We continued to do this for $ v^{*}_{3}, .. v^{*}_{12} $. This process produces a single covering for the set of vertices of interest. For any particular vertex, however, the covering set may include redundant representations according to the covering threshold. The set of unique representations found is not invariant to the order of the vertices nor the initialization of the set. 

To evaluate the proposed ILP we use the following scheme.
For each $(v^*,S^*)$ pair
we randomly partition $S^*$ ($|S^*|=20)$
into five subsets each of size four. These subsets are then each in turn used as $ S $ for the corresponding $ v^{*} $ and the ILP is evaluated on the remaining $|S^* \setminus S|=16$ vertices via MRR. This procedure resulted in a total of 15 different $ (v^{*}, S) $ pairs.
%used numerical Monte Carlo for each of the three $ v^{*} $. In particular, for each $ S^{*} $ we randomly partitioned the set of 20 elements into parts of size 4. These sets of 4 were then each used as $ S $ for the corresponding $ v^{*} $ and the ILP was evaluated on the remaining 16 vertices via $ MRR $. This procedure resulted in 15 different $ (v^{*}, S) $ pairs.


% need a set of vertices known to be similar to $ v^{*} $, or $ S $, and at least one other vertex known to be similar to $ v^{*} $ that is not in $ S $. In our analysis, we consider the set of pairs $ \{(v^{*}, S_{i})'\}_{i=1}^{|S|} $ found by leaving a single element of $ S $ out of $ S_{i}' $. That is, $ S_{i}' = S \setminus \{s_{i}\} $ with $ s_{i} \in S $. Given a $ (v^{*}, S_{i}') $ pair, the performance of the ILP is measured by where it places $ s_{i} $ in its nomination list. 
 
% Vertices represent particular products and edges are defined by [\textit{how are edges defined}]. Here, we start with a set of $ 12 $ vertices of interest. For each vertex of interest we are given a set of vertices known to be similar to it and a distance matrix from it to every other vertex in the network for $ J = 100 $ different distances. 

We compare the ILP to the nomination scheme that selects a ranker from the subset of the $ \{h^{d^{j}}\}_{j=1}^{100} $ that minimizes the objective function in \eqref{eq:main-prob}. That is, the second scheme uses the ranker induced by one of the $ 100 $ representations that minimizes the maximum rank of an element of $ S $. If two or more rankers tie then the ranker used is randomly selected from the argmin set. This scheme is referred to as ``Singleton" because it uses only a single representation.
Note that when a single representation optimizes \eqref{eq:main-prob} then the ILP and Singleton produce the same ranking.

The competing nomination schemes are, again, evaluated via MRR. The paired difference histogram and density estimate between the MRR from the ILP and the average MRR from Singleton are shown in Figure \ref{subfig:ip_minus_bing}. 
Testing the hypothesis ``$H_{0}$: Singleton is as good or better than ILP" results in $ p \approx 0.0003 $ from Wilcoxon's signed rank test.
(More to the point: ILP is {\it strictly} superior to Singleton for all 15 cases.)

% distances, or set of distances, that  two nomination schemes. Recall that nomination schemes have access to $ S $, a set of vertices known to be similar to the vertex of interest. The first scheme simply selects the metric that minimizes the maximum rank of an element of $ S $. That is, the metric that minimizes \ref{goal}. If two or more metrics tie then one of the metrics that tied is selected at random. This scheme is referred to as ``Singleton" in Figure \ref{fig:ip_minus_bing} because it uses a single metric. 

% The second scheme is the proposed IP. Note that the IP is the same as ``Singleton" if ``Singleton" places all of the elements of $ S $ at the top of it's nomination list. Otherwise, the integer program of Section \ref{subsec:IP} is used to find an optimal linear combination of distances. 

% Before evaluating the two nomination schemes, we first remove redundant metrics. In particular, if two metrics produced distances that were too similar, we remove one of them. Figure \ref{subfig:scree} shows the ordered $ 12 {100 \choose 2} $ pairwise distances. To decide what ``redundant" meant, we used an automatic elbow finding technique [ZG] and selected the second elbow. In this case the second elbow happened to be the last elbow. We were left with 15 metrics.



% HH:
% For each v* there are 100 different vectors of distances. I found all (100 choose 2) L2 norms of the differences for every v* (meaning 12 * (100 choose 2) total distances), ordered them and found all the elbows in the "scree" plot. 
% Then 
% The left panel of Figure 4 shows the ordered L2 norms of all the 12* (100 choose 2) differences. The vertical lines are the elbows found by ZG.

% Let $ v_{1}, .., v_{12} $ be a collection of vertices of interest and$  D_{v_i} $ for $ i \in {1, .., 12} $ be the personal distance matrix for vertex $ i $. That is, the $ jth $ column of $ D_{v_i} $ is the vector of distances from $ v_i $ to all other vertices in the graph as defined by distance $ j $.

% Let $ dist^{i}_{j,k} $ denote the L2 norm of the $ jth $ and $ kth $ vectors of distances corresponding to $ v_i $. Now consider the set of distances $ M = \{dist^{i}_{j,k}: i \in \{1, .., 12\}, j < k \in \{1, .., 100\}\} $. The left panel of Figure 4 shows the elements of M in descending order. The red lines show the elbows of the "scree" plot as found by ZG.

% The L2 norm corresponding to the second elbow of the scree plot was used as a threshold to recursively select "unique" distances. In particular, we initialized the set of unique distances with the first distance and subsequently selected distances where the L2 norm between it and every element in the set of unique distances was above the threshold for $ v_1 $. For $ v_2 $ the set of unique distances was initialized with the set found using $ v_1 $ and the process was repeated. We continued to do this for $ v_3, .. v_12 $. We note that the set of unique distances found is not invariant to the order of the vertices nor the initialization. 




% We evaluated the nomination schemes on 12 different $ v^{*} $. Each $ v^{*} $ had a corresponding set $ S_{v^{*}} $, ranging in size from 2 to 6. To evaluate the two schemes, we used a leave-one-out approach. That is, the nomination schemes had access to $ |S_{v^{*}} - 1 | $ of the elements of $ S_{v^{*}} $ and were then prompted to return the ranking of the remaining element of $ S $. In total, we had 47 $ (v^{*}, s^{*}) $ pairs. For 30 of these pairs, ``Singleton" and the IP produced the same nomination. 

% The paired difference histogram and estimated density for the remaining 17 pairs are shown in Figure \ref{fig:ip_minus_bing}.

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/bing/ip_minus_singleton_iphones_Ssize4_acorn1.pdf}
%     \caption{For nominating MBINs: histogram and estimated density of the paired difference of Mean Reciprocal Rank ($MRR$) between the ranker produced by the proposed integer program and a the ranker produced by choosing the best single distance. Each of the 26 MBINs in the connectome was considered $ v^{*} $. 15 of the remaining 25 MBINs were then chosen to be known similar vertices. The nomination schemes were evaluated on the final 10 MBINs. In this setting the effect size of the difference is quite large in favor of the ILP. Wilcoxon's one-sided signed rank test yields $ p \approx 0.0005 $.}
%     \label{fig:ip_minus_bing}
% \end{figure}

% \begin{figure}
%     \centering
%     \captionsetup[subfigure]{justification=centering}
%     \begin{subfigure}{0.49\columnwidth}
%         \includegraphics[width=\linewidth]{images/bing/paired_distance_scree.pdf}
%     %     \caption{}
%     %     \label{subfig:scree}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\columnwidth}
%         \includegraphics[width=\linewidth]{images/bing/ip_minus_vertices_ZG2_combined.pdf}
%     %     \caption{}
%     %     \label{subfig:ip_minus_bing}
%     \end{subfigure}
%     \caption{The proposed integer program is better than the collection of individual distances. Subfigure a) is the scree plot of the paired distances between distance vectors for all $ v^{*} $. Red lines indicate the "elbows" of the scree plot as detected by a profile likelihood ratio. Subfigure b) is the histogram and estimated density of the paired differences between the IP and the collection of all individual distances. The majority of the mass of the histogram is on the positive side of 0, indicating that the IP outperforms the collection of all individual distances. A signed-rank test for symmetry around 0 results in a p-value of 
%   % $ \approx 0.031 $.
%     $\approx 0.016$.
%     }
%     \label{fig:ip_minus_bing}
% \end{figure}

\begin{figure}[t]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\linewidth]{images/bing/ip_minus_singleton_iphones_Ssize4_acorn1.pdf}
        \caption{Bing}
        \label{subfig:ip_minus_bing}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\linewidth]{images/drosophila/ip_minus_singleton_mbins_Ssize15_acorn2.pdf}
        \caption{\textit{Drosophila}}
        \label{subfig:ip_minus_drosophila}
    \end{subfigure}
    \caption{For nominating phones and MBINs: histogram and estimated density of the paired difference of Mean Reciprocal Rank (MRR) between the ranker produced by the proposed integer program and the ranker produced by choosing the best single distance. \textit{Left}: Three different phones were considered to be a $ v^{*} $. Each phone has an associated $ S^{*} $ consisting of 20 elements. For each $ v^{*} $ we partition its corresponding $ S^{*} $ into 5 sets.
    We consider each set in a $ (v^{*}, S) $ pair. We evaluate the nomination schemes on the remaining 16 elements of $ S^{*} $.
    \textit{Right}: Each of the 26 MBINs in the connectome is considered $ v^{*} $. Of the remaining 25 MBINs, 15 are then chosen to be known similar vertices. The nomination schemes are evaluated on the remaining 10 MBINs. In both of these settings the effect size of the difference in MRR is quite large in favor of the ILP. Wilcoxon's signed rank test yields $ p \approx 0.0003$ (Bing, left) and $ p < 0.0001 $ (\textit{Drosophila}, right).}
    \label{fig:ip_minus_bing_and_drosophila}
\end{figure}

\subsection{Drosophila} We consider a synaptic-resolution connectome of the \textit{Drosophila} larva brain (unpublished), including its learning and memory center (the mushroom body) 
% We consider a fully mapped connectome of a \textit{Drosophila} larva 
\cite{eichler2017complete}. The connectome consists of $ n = |V| = 2965 $ neurons.
% and includes neurons from both the left and right hemispheres. 
Edges are synapses -- directed. There are four edge types in the connectome: axon to dendrite $(|E_{AD}| = 54303)$, axon to axon $(|E_{AA}| = 34867)$, dendrite to dendrite $(|E_{DD}| = 10209)$, and dendrite to axon $ (|E_{DA}| = 4088)$. This connectome was manually annotated from electron microscopy imagery for a single \textit{Drosophila} larva brain \cite{ohyama2015multilevel, schneider2016quantitative}.

The four different edge types possibly contain different and complementary information for inference related to neuron types in the connectome. This information is likely more useful than a single summary edge weight, such as the sum of the edge weights across the four different edge types.

We consider $J=4$ different representations of the connectome obtained via spectral embedding of the individual Laplacian matrices corresponding to the four different directed weighted edge types. 
%The omnibus matrix \cite{levin2017central} is the $ 4n \times 4n $ matrix with the individual Laplacian matrices on the block diagonal and their pairwise averages in the off-block diagonals.

% Rewrite 
These spectral embeddings yield a representation of each node for each edge type.
%in the same Euclidean space. 
Note that since the connectome is directed, the left and right singular vectors differ. We use the concatenation of the two (embedding dimension $ m=11 $) as the representation, resulting in a $ 22 $ dimensional representation for each neuron for each edge type.  

%The other four representations are found by spectrally embedding (embedding dimension $ m=11 $) a transformation of the omnibus matrix that is analagous to LSE in the multigraph setting.
%We again use the concatentation of the left and right scaled singular vectors as the representation for each neuron for each edge type.

The input neurons of the mushroom body (MBINs) are a well known and studied neuron type within the \textit{Drosophila} larva connectome \cite{saumweber2018functional}. For illustration purposes we consider each of the 26 MBINs in the brain as a $ v^{*} $ and 15 randomly selected MBINs as vertices known to be similar to $ v^{*} $. We evaluate the ILP and Singleton via MRR on the remaining 10 MBINs. Recall that Singleton uses a ranker from amongst the single representations that minimizes the objective function in \eqref{eq:main-prob}.

The paired difference histogram and estimated density between the MRR from the ILP and the MRR from Singleton are shown in Figure \ref{subfig:ip_minus_drosophila}. Testing the hypotheses ``$H_{0}$: Singleton is as good or better than ILP" results in $ p < 0.0001 $. This result indicates that the different edge types contain complimentary information that, when put together, can yield superior inferential procedures as compared to procedures using only a single edge type. 

Of particular interest is the breakdown of solutions in terms of edge type.
As an example,
in one representative trial
the best singleton is AA (axon-to-axon),
while the ILP solution is the linear combination
of (AA,AD,DA,DD)
with weights (0.424, 0.123, 0, 0.453).
Indeed:
the Singleton solution is always one of AA,AD,DD -- never DA,
and the ILP solution is always a linear combination of just these three edge types.




%{\color{red} should we mention that the results are highly correlated?}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/drosophila/ip_minus_singleton_mbins_S15.pdf}
%     \caption{For nominating MBINs: histogram and estimated density of the paired difference of Mean Reciprocal Rank ($MRR$) between the ranker produced by the proposed integer program and a the ranker produced by choosing the best single distance. Each of the 26 MBINs in the connectome was considered $ v^{*} $. 15 of the remaining 25 MBINs were then chosen to be known similar vertices. The nomination schemes were evaluated on the final 10 MBINs. In this setting the effect size of the difference is quite large in favor of the ILP. Wilcoxon's one-sided signed rank test yields $ p \approx 0.0005 $.}
%     \label{fig:ip_minus_drosophila}
% \end{figure}



















% why did we not use all 100 distances?

% one reason why MSR might care


% from the collection of graphs  graphs a single diffusion MRI from the dataset considered in TT@PNAS. In particular, we chose 1 of 114 connectomes 

% a single diffusion MRI from a collection of 114 connectomes 


% - What is it? (brain data; part of a larger collection of brain data;  
% - 

% This dataset was used to show the two truths phenomenon in spectral clustering.

% In the analysis below we consid

% We consider for illustration a diffusion MRI dataset consisting of 114 connectomes (57 subjects, two scans each) with 72,783 vertices each and both left/right/other hemispheric and gray/white/other tissue attributes for each vertex. Graphs were estimated using the NeuroData’s MR Graphs pipeline (23), with vertices representing subregions defined via spatial proximity and edges defined by tensor-based fiber streamlines connecting these regions (Fig. 2).

% The actual graphs we consider are the largest connected component (LCC) of the induced subgraph on the vertices labeled as both left or right and gray or white. This yields m=114 connected graphs on n≈40,000 vertices. Additionally, for each graph every vertex has a {Left,Right} label and a {Gray,White} label, which we sometimes find convenient to consider as a single label in {LG,LW,RG,RW}.


